Learning Motion Predictors for Smart Wheelchair using Autoregressive Sparse Gaussian Process

Constructing a smart wheelchair on a commercially available powered wheelchair (PWC) platform avoids a host of seating, mechanical design and reliability issues but requires methods of predicting and controlling the motion of a device never intended for robotics. Analog joystick inputs are subject to black-box transformations which may produce intuitive and adaptable motion control for human operators, but complicate robotic control approaches; furthermore, installation of standard axle mounted odometers on a commercial PWC is difficult. In this work, we present an integrated hardware and software system for predicting the motion of a commercial PWC platform that does not require any physical or electronic modification of the chair beyond plugging into an industry standard auxiliary input port. This system uses an RGB-D camera and an Arduino interface board to capture motion data, including visual odometry and joystick signals, via ROS communication. Future motion is predicted using an autoregressive sparse Gaussian process model. We evaluate the proposed system on real-world short-term path prediction experiments. Experimental results demonstrate the system's efficacy when compared to a baseline neural network model.

==> sections/experiment/generate_examples.tex <==

In this section, we discuss how to convert the joystick and velocity sequences into a set of input-output pairs for training the regression models (Eq. \ref{eq:mainauto}). Furthermore, convert the sequences into pose trajectories for validating the performance of the pose trajectory prediction. 

For \textit{linear immediate prediction} (Eq. \ref{eq:linear_imm}), consider a linear sequence $\{(j_i, v_i)\}_{i = 1 \cdots n}$. We convert the sequence into a set of $n$ input-output pairs by
\begin{align}
&\{(X_i, v_i)\}_{i=1 \cdots n}\label{eq:imm_pair}  \\
&X_t = [j_{t-s}, \cdots, j_{t-2}, j_{t-1}, v_{t-s}, \cdots, v_{t-1}, j_t]^T\nonumber
\end{align}
where $v_i$ is the linear velocity at time-step $i$. Afterward, the $n$ input-output pairs are used to train our regression models that implements Eq. \ref{eq:linear_imm}. The same procedure is used to train the angular velocity models (Eq. \ref{eq:angular_imm}). In the pose trajectory prediction phase, we use the trained models with Algorithm \ref{alg:k_predict} to predict a velocity sequence and then integrate the sequence into a pose trajectory. 

To generate the inputs for motion predictors and to validate their performance in pose trajectory prediction, the corresponding pose trajectory test cases need to be generated.
Given $\{(j_i, v_i)\}_{i = 1 \cdots n}$, the linear part of the test sequence, we convert it into $n$ input-output pairs by:
\begin{align}
&\{(Z_i, Y_i)\}_{i=1 \cdots n}\label{eq:traject_pair}\\
&Z_t = [j_{t-s}, \cdots, j_{t+(k-1)}, v_{t-s}, \cdots, v_{t-1}]^T\nonumber\\
&Y_t = [v_{t}, v_{t+1},\cdots, v_{t+(k-1)}]^T\nonumber
\end{align}
where $Z_t$ is the input and $Y_t$ is output for predicting linear velocity sequence using a one-dimensional version of Algorithm \ref{alg:k_predict}.
We apply the same conversion for the angular part of the test sequence and use the $n$ sequences for the linear version and the angular version of $Y_t$ to obtain the corresponding pose trajectories by the integration procedure (Eq. \ref{eq:recur_sol}). 

An obvious question is how to deal with the boundary cases in the dataset in which either the past $s$ steps of the time series or the future $k$ steps of joystick sequence is not present. It can be easily resolved by having the robot not moving at the beginning and the ending of our dataset, which implies that we could zero the joystick inputs as well as the velocity outputs for the boundary case. Furthermore, having the robot not moving, we can reasonably assume that each collected sequence is independent of each other, which implies that we could append the sequences at arbitrary order to train and test our models.




==> sections/methodology/pose_traject.tex <==
Suppose a velocity sequence $\{V_i\}_{i=1 \cdots k} = \{(v_i, w_i)\}_{i=1 \cdots k}$ is given, we want to obtain the corresponding pose trajectory $\{P_i\}_{i=1\cdots k} = \{(x_i, y_i,\theta_i)\}_{i=1\cdots k}$. The Unicycle Model (Fig. \ref{fig:unicycle_model}) can be used to model the relationship between the two as differential equations:
\begin{equation*}\label{eq:unicycle_de}
u=\begin{bmatrix}
\dot{x}\\ 
\dot{y}\\
\dot{\theta} 
\end{bmatrix}
=\begin{bmatrix}
v cos\theta\\ 
v sin\theta\\ 
\omega
\end{bmatrix}
\end{equation*}
which can be solved by integration. 
\begin{gather*}\label{eq:int_omega}
\left\{\begin{aligned}
x(t) &= \int_{0}^{t}v(s)cos(\theta(s))ds \\
y(t) &= \int_{0}^{t}v(s)sin(\theta(s))ds \\
\theta(t) &= \int_{0}^{t}\omega(s)ds 
\end{aligned}\right.
\end{gather*}
Since the quantities are sequences of data, numerical integration is used. The recurrence relations for the integration are the following (assuming the points are equally meshed with width $h$):
\begin{align}\label{eq:recur_sol}
\theta_i &= \begin{cases}
\theta_{i-1} + \frac{h}{2} (w_{i-1} +w_{i}) \text{, if } i > 1\\
\pi/2 \text{, otherwise}
 \end{cases}
\\
x_{i} &= \begin{cases} 
 x_{i-1}+   \frac{h}{2} (v_{i-1}cos(\theta_{i-1}) +v_{i}cos(\theta_{i})) \text{, if } i > 1\\
0\text{, otherwise}\nonumber
\end{cases}
\\
y_{i} &= \begin{cases} 
 y_{i-1}+   \frac{h}{2} (v_{i-1}sin(\theta_{i-1}) +v_{i}sin(\theta_{i})) \text{, if } i > 1\\
0\text{, otherwise}\nonumber
\end{cases}
\end{align}
Note that we define the initial pose of the robot as $(0, 0, \pi/2)^T$, which implies the robot sits at the origin and heads to the direction of the positive side of the y-axis.

An example of derivation for the integration procedure using the trapezoidal rule is provided:
\begin{align*}
\theta_{i+1} &= \theta_i + \int_{t_{i}}^{t_{i+1}} \omega(s) ds \\
&\approx \theta_i + \frac{h}{2} (w(t_i) +w(t_{i+1}))\nonumber \\
&= \theta_i + \frac{h}{2} (w_i +w_{i+1})\nonumber
\end{align*}





==> sections/methodology/slide_window.tex <==
One common method to convert a sequential supervised learning method into a classic regression problem is the Recurrent Sliding Window Method \cite{dietterich2002machine}. Similar to the Sliding Windows Method, to predict a target $y_t$ at time t, it only uses the input through a window of size $d$ centered at $t$. For example, to predict $y_t$, it uses the input on a window $[x_{t-d}, x_{t-d+1}, \cdot, x_t, \cdots, x_{i+d-1}, x_{t+d}]$ from the input sequence $\textbf{x}$. Different from the Sliding Window Method, the Recurrent Sliding Window Method appends the past $d$ predictions, $\hat{y_{t-d}}, \hat{y_{t-d+1}},\cdots, \hat{y_{t-2}},\hat{y_{t-1}}$ into the input window $[x_{t-d}, x_{t-d+1}, \cdot, x_t, \cdots, x_{i+d-1}, x_{t+d}]$ to predict $y_t$. 

As a result, given an input and the corresponding output sequence $\{(x_i,y_i)\}_{i=1\cdots N}$, for each $i$ we construct a window for the target $y_i$, which leads to N training examples from two size N sequences. Notably, the method cannot create windows at the boundaries of the sequences. For example, at time 1, there are no input and output sequences on the left side of the window. Therefore, we constrain our robot to be at rest at the beginning and the end of the sequences so that zeros can be used for the out-of-bound windows.
